Towards Zero-Shot Multilingual Synthetic Question and Answer Generation for Cross-Lingual Reading Comprehension

We propose a simple method to generate multilingual question and answer pairs on a large scale through the use of a single generative model. These synthetic samples can be used to improve the zero-shot performance of multilingual QA models on target languages. Our proposed multi-task training of the generative model only requires the labeled training samples in English, thus removing the need for such samples in the target languages, making it applicable to far more languages than those with labeled data. Human evaluations indicate the majority of such samples are grammatically correct and sensible. Experimental results show our proposed approach can achieve large gains on the XQuAD dataset, reducing the gap between zero-shot and supervised performance of smaller QA models on various languages.

==> Multilingual QAGen/acknowledgement.tex <==
\section{Acknowledgement}\label{sec:acknowledgement}
We  thank Fadi Haik, Nizar Saqqar, Bahaa El-Taweal, Stanela Khalil, Igor Krivokon, Vladimir Magay, Tania Rojas-Esponda, and Gustavo Hernandez Abrego for  evaluations of the samples and providing valuable feedback on their quality.

==> Multilingual QAGen/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In this work, we presented a simple yet effective approach to generate large-scale synthetic multilingual question-answer pair data, which can be used to improve the zero-shot performance of multilingual RC models. Our experimental results showed large improvements in the performance of RC models trained on our synthetic multilingual datasets as compared to standard zero-shot baselines. Moreover, our zero-shot generation approach proved to be easily applied to any language, as long as the language is supported by the pre-trained multilingual generative model.

While our results showed that using synthetic samples alongside English training data can significantly narrow the gap between zero-shot and supervised performance of RC models, the gap still remains. We are optimistic that future work can reduce this gap further through improved generation quality.

==> Multilingual QAGen/experiments.tex <==
\section{Experimental Setup and Results}\label{sec:experiments}

% \begin{table}[]
% \centering
% \footnotesize
% \scalebox{0.90}{
% \begin{tabular}{l|lllllll} \hline
% Task          & AR  & DE   & EN   & ES  & HI  & VI   & ZH  \\ \hline
% QA Generation & 1.7 & 3.0  & 23.4 & 3.6 & 3.2 & 4.4  & 1.2 \\
% Co-Training & \textbf{6.8} & \textbf{12.3} & \textbf{24.9} & \textbf{9.5} & \textbf{8.2} & \textbf{11.1} & \textbf{4.6} \\ \hline
% \end{tabular}
% }
% \caption{{\small Performance of question generation on the MLQA test set with mT5-XL.}}
% \label{qgen}
% \end{table}


% \begin{table}[]
% \centering
% \footnotesize
% \scalebox{0.92}{
% \begin{tabular}{l|lllllll} \hline
% Model Size     & AR  & DE   & EN   & ES  & HI  & VI   & ZH  \\  \hline
% Base (600M)  & 2.1 & 6.3  & 22.3 & 4.8 & 5.2 & 6.9  & 2.2 \\ 
% Large (1B) & 3.3 & 9.3  & 23.9 & 5.7 & 4.8 & 8.0  & 2.4 \\
% XL (4B)   & \textbf{6.8} & \textbf{12.3} & \textbf{24.9} & \textbf{9.5} & \textbf{8.2} & \textbf{11.1} & \textbf{4.6} \\ \hline
% \end{tabular}
% }
% \caption{{\small Performance of question generation (co-training setting) on the MLQA test set for different mT5 model sizes.}}
% \label{qgen-size}
% \end{table}

% \begin{table*}[]
% \centering
% \footnotesize
% \scalebox{0.92}{
% \begin{tabular}{l|ccccccccccccccccccc}
% \hline
% \multirow{2}{*}\textbf{Dataset} & \multicolumn{2}{c}{\textbf{ES}} & \multicolumn{2}{c}{\textbf{DE}} & \multicolumn{2}{c}{\textbf{AR}} &
% \multicolumn{2}{c}{\textbf{HI}} & \multicolumn{2}{c}{\textbf{VI}} & \multicolumn{2}{c}{\textbf{ZH}} \\ 
% & EM & F1 & EM & F1 & EM & F1 & EM & F1 & EM & F1 & EM & F1 \\
% \hline
% SQuAD en  & 57.06 & 74.62 & 55.55 & 71.46 & 43.28 & 60.26 & 44.62 & 59.21 & 50.84 & 70.66 & 50.59 & 59.07\\ 
% Synthetic only & 57.90 & 75.43 &54.79 & 72.06 & 45.38 & 62.57 & 46.13 & 62.57 & 49.33 & 68.25 & 42.86 & 58.70\\
% SQuAD en + Synth. & \textbf{60.50} & \textbf{78.50} & \textbf{59.41} & \textbf{75.36} & \textbf{49.33} & \textbf{66.00} &\textbf{50.17} & \textbf{66.24} &\textbf{53.45} & \textbf{73.12} & \textbf{52.27} & \textbf{63.32}\\ 
% \hdashline
% \textit{Supervised} & 63.87 & 80.61 & 62.10 & 76.99 & 54.79 & 70.85 & 56.13 & 70.86 & 58.57 & 77.35 & 58.99 & 67.02\\
% \hline
% \end{tabular}
% }
% \caption{{\small Performance of fine-tuned mBERT models on XQuAD. \textit{Supervised} refers to training on SQuAD en + \texttt{translate-train} dataset of the target language.}}\label{tab:xquad}
% \end{table*}

% \begin{table*}[]
% \centering
% \footnotesize
% \scalebox{0.92}{
% \begin{tabular}{l|ccccccccccccccccccc}
% \hline
% \multirow{2}{*}\textbf{Dataset} & \multicolumn{2}{c}{\textbf{ES}} & \multicolumn{2}{c}{\textbf{DE}} & \multicolumn{2}{c}{\textbf{AR}} &
% \multicolumn{2}{c}{\textbf{HI}} & \multicolumn{2}{c}{\textbf{VI}} & \multicolumn{2}{c}{\textbf{ZH}} \\ 
% & EM & F1 & EM & F1 & EM & F1 & EM & F1 & EM & F1 & EM & F1 \\
% \hline
% SQuAD en &47.42 & 65.10 & 44.65 & 59.62& 33.06 & 51.27 & 34.83 &50.30 &41.53 & 61.51 &38.70 & 59.14\\ 
% Synthetic only &48.81 & 67.58 & 46.96 & 63.17 & 35.50 & 54.62 &40.02 & 58.01 &42.88&63.15 &34.55 & 59.20\\
% SQuAD en + Synth. &\textbf{51.70}&\textbf{70.32} & \textbf{49.63} & \textbf{65.21} &\textbf{37.71}& \textbf{56.48} & \textbf{42.94}& \textbf{59.96} & \textbf{46.02}& \textbf{66.79}  & \textbf{42.20}& \textbf{64.19}\\ 
% \hdashline
% \textit{Supervised} & 52.90 & 70.74 & 51.36 & 65.86 & 38.76 & 57.88 & 45.69 & 62.72 & 47.28 & 67.57 & 43.84 & 65.98 \\
% \hline
% \end{tabular}
% }
% \caption{{\small Performance of fine-tuned mBERT models on MLQA test set. \textit{Supervised} refers to training on SQuAD en + \texttt{translate-train} dataset of the target language.}}\label{tab:mlqa}
% \end{table*}


\subsection{Datasets}
\textbf{SQuAD} \cite{squad} is an English QA dataset consisting of 100k samples. The passages are extracted from Wikiepdia. We use the train and dev splits of SQuAD 1.1 in this work. \\
\textbf{XQuAD} \cite{xquad} is a multilingual QA dataset consisting of 240 paragraphs and 1190 question-answers in Arabic, Chinese, German, Greek, Hindi, Russian, Spanish, Thai, Turkish and Vietnamese. These samples have been professionally translated from the SQuAD 1.1 dev set. \\
\textbf{MLQA} \cite{mlqa} is a benchmark dataset for evaluating cross-lingual question answering performance. This dataset contains over 5k QA instances (12k in English) following the SQuAD format in each of Arabic, Chinese, English, German, Hindi, Spanish and Vietnamese. We use the test split in our evaluations.\\ 
\textbf{TyDiQA} \cite{tydiqa} is another multilingual QA dataset consisting of 200k QA pairs from 11 typologically diverse languages. There is less lexical overlap between questions and answers compared to XQuAD and MLQA. We use the Gold Passage task, which includes \textasciitilde 50k samples in the train split and between 130 and 1100 samples for each language in the development set. % The development set of the Gold Passage task, which includes between 130 and 1100 samples in each target language. The Gold Passage training set includes \textasciitilde 50000 samples.

% With XQuAD and TyDiQA, we utilized the official SQuAD 1.1 evaluation script to calculate the metrics. With MLQA, we used the official task evaluation script, as instructed by the task guidelines.

\textbf{XTREME} \cite{xtreme} is a multilingual benchmark consisting of nine tasks spanning 40 typologically diverse languages. This dataset includes machine translated SQuAD 1.1 train and dev samples, which we employed in our experiments. We refer to such samples as \texttt{translate-train}.
\subsection{Generative Model Fine-tuning}\label{sec:genfine-tuning}
We used the official mT5-XL model \cite{mt5} with 3.7 billion parameters as the generative model. The official pre-trained checkpoint is fine-tuned using the mixture of tasks described in section~\ref{sec:modeling}. We chose the task mixing ratio to be 10:1, meaning for every 10 instances of the QA Generation task (\ref{sec:qa_gen_task}), we mix one instance of the MLM task (\ref{sec:mlm}). We experimented with other mixing ratios of 1000:1 and 100:1, as well, all of which under-performed 10:1.
The unsupervised MLM task covers text from two domains: 1) the subset of the mC4 corpus \cite{mt5} covering Arabic, Bengali, English, Finnish, Indonesian, Korean, Russian, Swahili, and Telugu, 2) questions from TyDiQA \cite{tydiqa} train and dev sets, covering the same set of languages. %Note that this is the MLM task used during our co-training, not to be confused with the original pre-training MLM task performed over 100 languages for mT5.

It is worth highlighting that we only fine-tune a single model to generate across all target languages. We do not apply language code prompts during fine-tuning or inference. We observe that by properly designing the fine-tuning mixture, the model is capable of generating samples in the language of the input passage. Human evaluations in section~\ref{sec:human-evals} further verify this.

All of our models are fine-tuned for 5000 steps with a batch size of 131,072 tokens, distributed over 64 TPU-v3 chips. The final checkpoint is used to perform synthetic data generation.

% \begin{table*}[]
% \centering
% \footnotesize
% \scalebox{0.92}{
% \begin{tabular}{l|ccccccccccccccccccc}
% \hline
% \multirow{2}{*}\textbf{Dataset} & \multicolumn{2}{c}{\textbf{AR}} & \multicolumn{2}{c}{\textbf{RU}} & \multicolumn{2}{c}{\textbf{FI}} & \multicolumn{2}{c}{\textbf{TE}}\\ 
% & EM & F1 & EM & F1 & EM & F1 & EM & F1\\
% \hline
% SQuAD en &45.39& 60.93 & 40.52 & 63.07 & 45.27 & 58.91 & 45.44 & 53.73  \\ 
% Synthetic only &\textbf{56.35}& \textbf{71.85}& \textbf{40.52}& \textbf{67.09} & 62.28 & 74.44 & \textbf{46.04} & \textbf{59.12}  \\
% SQuAD en + Synth. &55.81& 71.52 & \textit{39.66}& \textit{66.70} & \textbf{62.79} & \textbf{74.74} & 45.44 & 54.58 \\
% \hdashline
% \textit{Supervised} & 67.75 & 82.46 & 59.36 & 76.03 & 69.69 & 80.65 & 70.55 & 84.74 \\
% \hline
% \end{tabular}
% }
% \caption{{\small Performance of fine-tuned QA models on TyDiQA Gold Passage task. \textit{Supervised} refers to train on TyDiQA Gold Passage training data.}}\label{tab:tydiqa}
% \end{table*}

\subsection{Automatic Evaluation Results}

To compute automatic metrics such as BLEU against QA samples of the development set, we modify the generation task to generate a question given the passage and the answer. Conditioning on the answer is needed, as without it, the generative model might generate samples that are of high quality but not related to the answers provided in the development set for a given passage. This would lead to inaccuracies in interpreting metrics such as BLEU\footnote{All BLEU scores in this work are calculated using SacreBLEU v1.3.0 \cite{post-2018-call}, with ``exp'' smoothing and ``intl'' tokenization.}. 

\input{qgen}
\input{qgen_size}

Tab.~\ref{qgen} compares BLEU performance of two fine-tuning settings on the MLQA test set. We report results using the mT5-XL model. As can be seen, including the MLM tasks has a large impact on performance, conveying large gains up to +15 absolute BLEU points. This is in line with our observations from section~\ref{sec:filtering}, where adding MLM fine-tuning task enabled the generative model to produce QA samples in the language of the target passage. 

Interestingly, MLM on either mC4 or TyDiQA questions results in similar BLEU scores. Furthermore, adding a mixture of two does not yield any extra gains. However, eyeballing the generated samples indicated that the model fine-tuned on the mixture of both MLM tasks and the supervised English task generates more well-structured and sensible questions and answers. Human evaluations in section~\ref{sec:human-evals} verify the high quality of generated samples from a model trained with this mixture.

To investigate the effect of the generative model size on the quality of data generation, we perform experiments using  mT5 variants with different number of parameters: Base (600M), Large (1B) and XL (3.7B). We report results of the fine-tuned models with the mixture setting (\ref{sec:multi-task}) on the MLQA dataset in Tab.~\ref{qgen-size}. Model performance improves dramatically with the size of the pre-trained model. Based on these results, for the remainder of the paper, we use the mT5-XL model fine-tuned using the mixture approach.

\subsection{Human Evaluations}\label{sec:human-evals}

To perform manual quality evaluation of the generated questions, raters were presented with generated questions, and tasked with rating them according to the following criteria: 
\begin{itemize}[noitemsep]
    \itemsep0em 
    \item \textit{Is the question in the target language?} Raters could select \textit{yes} or \textit{no}.
    \item \textit{grammatical correctness:} Raters could select a whole number from 1 (lowest) to 4 (highest). 
    \item \textit{sensibility:} Raters could select a whole number from 1 (lowest) to 4 (highest). 
\end{itemize}
% For the second task, raters were presented with a generated question and answer alongside the passage that they were generated from. The raters were asked how accurate the generated question and answer are w.r.t the passage. They could select from 1 (lowest) to 4 (highest). 

In total, 400 generated samples from 5 languages were randomly selected and rated by native speakers of each language. Each rater was assigned 40 samples. Two native speakers of each of the five languages were asked to perform the task. Tab.~\ref{tab:human_evals} shows the evaluation results. 

The results show that the multilingual generative model is nearly perfect at generating samples that match the language of the input passage. Considering no language codes are used during fine-tuning, and only the English supervised training data was used, the results show that our proposed mixture has enabled the model to perform zero-shot cross-lingual generation coherently.

Interestingly, Spanish samples achieve high scores in all of the categories. Considering the model is not trained on any Spanish samples, either in the MLM tasks or SQuAD~1.1, the model shows strong transfer learning capabilities. This implies that including the MLM task as proposed in our mixture setting not only prevents the generative model from \textit{catastrophic forgetting} of its multilingual capability on the languages included in the MLM fine-tuning task, but also on those not included.
The same argument partially applies to Hindi. While there are no Hindi samples in the fine-tuning mixture, Bengali (a related Indo-Aryan language) was seen in the MLM task.

\input{human_evals}


\section{Application of Synthetic Data to Multilingual Reading Comprehension}\label{sec:downstream_experiments}
In this section, we describe experimental results that demonstrate the efficacy of using synthetic samples for improving multilingual reading comprehension models. RC refers to the setting where given a passage and a question, the model is tasked with finding a span of the passage that answers the question.

\subsection{Synthetic Data Generation}\label{sec:synthgen}

We randomly selected 10k paragraphs from Wikipedia \cite{wikidump}, for each of Arabic~(ar), German~(de), Hindi~(hi), Russian~(ru) and Spanish~(es). The selected paragraphs were restricted to have between 30 and 450 tokens, thereby removing passages that are too long or too short.

We fine-tune the mT5-XL model according to the mixture setting discussed in section \ref{sec:multi-task} and the hyper-parameters from section \ref{sec:genfine-tuning}, and then use this model to generate 20 questions per passage. \textit{Top-k} sampling \cite{holtzman2020curious} with \textit{k=10} and temperature of 0.5 was applied. The generated samples are processed to ensure: 1) each consists of a question followed by an answer, 2) the answer does exist in the passage. This was done to ensure answers are extractive. Non-extractive or no-answer QA are outside the scope of this work.

As discussed in section \ref{sec:filtering}, round-trip filtering is applied to the generated QA samples. We used an mT5 XL model trained on SQuAD 1.1 \cite{squad11} as the filtering model. This process would result in approximately 10-20k synthetically generated samples per each target language. The generated samples are used in training the RC models.

\subsection{RC Model Fine-tuning}
All our reading comprehension models are initialized from the official mT5 \cite{mt5} and later fine-tuned on the generated samples. We experimented with Base (580M), Large (1.2B), and XL (3.7B) parameter variants of mT5. We fine-tune using the TensorFlow framework. Each model was trained for \textit{10000} steps with a learning rate of \textit{1e-3} and a batch size of \textit{131072} tokens. The models were trained on 16 TPU-v3 chips.
In experiments where both the SQuAD 1.1 samples and synthetically generated ones are used to fine-tune the RC models, the model is trained on a mixture of the two, with a mixing ratio of \textit{1}. 

\subsection{Results}
% \input{xquad}
% \input{mlqa}
% \input{tydiqa}
\input{xquad_mt5_base}
Tabs.~\ref{tab:xquad_mt5_base}--\ref{tab:xquad_mt5_xl} demonstrate the F1 performance of the RC models trained on SQuAD 1.1 samples as well as synthetic data generated as described in \ref{sec:synthgen} on mT5 Base, Large, and XL models. ``\textit{SQuAD en}'' refers to the original SQuAD~1.1 \cite{squad11} dataset in English. Our zero-shot baselines, denoted by \textit{(ours)} were slightly higher than those reported in \cite{mt5} \textit{(paper)}. %``\textit{Supervised}'' refers to training with a mixture of SQuAD~1.1 and \texttt{translate-train} dataset of the target language.

% In Tabs.~\ref{tab:xquad_} and \ref{tab:mlqa}, ``\textit{Supervised}'' refers to training on SQuAD en + \texttt{translate-train}. In Tab.~\ref{tab:tydiqa}, ``\textit{Supervised}'' refers to training on TyDiQA Gold Passage training data \cite{tydiqa}. \textbf{Bold} indicates the best values overall for each target language, excluding the supervised setting.

% The following can be observed: 1)~Augmenting \textit{SQuAD en} with synthetic samples always leads to improvements in the performance of the RC models across all languages and all datasets. On Hindi MLQA, more than \textbf{+8/+9} absolute point improvements in EM/F1 scores are observed. 2)~For all TyDiQA languages and all MLQA languages except Chinese, the models trained with synthetic samples only outperform those trained with \textit{SQuAD~en} only. Similarly, on XQuAD, the performance of synthetic samples alone is either better or within a few points of \textit{SQuAD en} (except Chinese). This observation points to the efficacy of using synthetic samples. 3)~On MLQA and XQuAD, across all languages, synthetic samples and \textit{SQuAD en} provide complementary gains. However this does not apply to TyDiQA, where adding \textit{SQuAD en} barely leads to any performance improvements. We hypothesize this is because on TyDiQA, the RC models trained on synthetic data alone outperform the \textit{SQuAD en} baseline by a large margin, e.g.~\textbf{+11/+11} absolute improvements on EM/F1 scores in Arabic. Such a gap indicates that \textit{SQuAD en} samples are less effective than synthetic in-domain samples in improving the performance on TyDiQA.
\input{xquad_mt5_large}
We can observe that ~Augmenting \textit{SQuAD en} with synthetic samples leads to large gains with the base model. \textbf{+9} absolute point improvement can be observed with Russian. Furthermore, with the base model, all the average F1's are improved with the addition of synthetic data, regardless of which language the synthetic samples come from. The largest gain is seen when German samples are added \textbf{(+2.9)}.

As the number of parameters of the mT5 model increases, the gains through synthetic augmentation become less, as results show in Tabs.~\ref{tab:xquad_mt5_large} and \ref{tab:xquad_mt5_xl}. The maximum average F1 improvements of \textbf{+1.2} absolute points with the Large model is achieved. With the XL model, the average F1 scores are either the same as the zero-shot baseline or slightly lower. This is expected as the model size increases, the gap between zero-shot and supervised also becomes smaller, hence less headroom exists when adding the synthetic samples. Fig.~\ref{fig:scaling_effect} demonstrates this scaling effect. Nonetheless, improvements of \textbf{+5.1}, \textbf{+2.2}, and \textbf{+3.4} are observed on Russian, Arabic, and Greek, respectively with the mT5 Large model. Similarly, smaller per language gains can be seen with augmentation with the XL model, as shown in Tab.~\ref{tab:xquad_mt5_xl}.
\input{xquad_mt5_xl}

%A surprising observation is that best per language results are not necessarily achieved when augmenting with the synthetic samples from the same target language. Our hypothesis is that strong multi-lingual models such as mT5 have already developed rich per language representations. Adding non-English synthetic data enables the model to generalize well to non-English RC tasks by not overfitting to English RC samples. 

Comparing the \textit{Supervised} metrics vs.~\textit{SQuAD en + <lang>.}\ indicates that using synthetic samples reduces the gap between the zero-shot versus supervised performance of the trained RC models with Base and Large. This gap is reduced from \textbf{7.2} to \textbf{4.2} absolute points with the base model. However, there still exists a sizeable gap, which can be further close with using higher quality synthetic samples. 

%One point we would like to highlight is that our proposed zero-shot synthetic data generation not only works well for high resource languages like Spanish or German, but can also be applied fruitfully to low resource languages like Telugu, where an over +5 point F1 improvement is observed on TyDiQA dev. 

% As discussed in \ref{sec:genfine-tuning}, the MLM task of co-training is only done on Arabic, English, Spanish, German, Vietnamese, Hindi and Chinese. Although Russian, Finnish and Telugu are not included in the MLM task, the fine-tuned generative model is still capable of generating samples in those languages, leading to large gains in the zero-shot performance of the RC models, as demonstrated in Tab.~\ref{tab:tydiqa}. Therefore, including the MLM task as proposed in co-training not only prevents the generative model from \textit{catastrophic forgetting} of its multilingual capability on the languages included in the MLM fine-tuning task, but also on those not included.
% Although Spanish is not included in the MLM task, as discussed in \ref{sec:genfine-tuning}, the fine-tuned generative model is still capable of generating samples in Spanish \textbf{CHECK IF THERE ARE OTHERS.}. Therefore, including the MLM task as proposed in mixture setting not only prevents the generative model from \textit{catastrophic forgetting} of its multilingual capability on the languages included in the MLM fine-tuning task, but also on those not included.

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.12]{f1_avg_comparison.png}
    \caption{\small{Scaling effect on augmentation using synthetic samples.}}
  \label{fig:scaling_effect}
\end{figure}

==> Multilingual QAGen/human_evals.tex <==
% \begin{table}[]
% \centering
% \footnotesize
% \scalebox{0.9}{
% \begin{tabular}{l|lll|l} \hline
% & \multicolumn{3}{|c|}{Questions} & \multicolumn{1}{|c}{QAs}  \\ \hline
% Metric     & Target & Grammatical  & Sensibility  & Accuracy  \\ 
% & Language & Correctness & &  \\
% \hline
% Russian & 1 & 3.5 & 3.75 & 3.2 \\
% Spanish & 1 & 3.1 & 3.05 & 2.85  \\
% Arabic & .98 & 3.55 & 3.35 & 2.3  \\
% Chinese & 1 & 3.6 & 3.6 & 3 \\
% Hindi & 1 & 2.93 & 3.35 & 3 \\ \hline
% Average & 1 & 3.34 & 3.38 & 2.87 \\
% \hline
% \end{tabular}
% }
% \caption{{\small Human Evaluation metrics on the generated samples. Samples are randomly drawn, and rated by the native speakers of Russian, Spanish, Arabic, Chinese, and Hindi.}}
% \label{tab:human_evals}
% \end{table}

\begin{table}[]
\centering
\footnotesize
\scalebox{0.9}{
\begin{tabular}{l|rrr} \hline

& Target & Grammatical  &   \\ 
& Language & Correctness & Sensibility \\
\hline
Arabic & 0.98 & 3.55 & 3.35   \\
Chinese & 1.00 & 3.60 & 3.60  \\
Hindi & 1.00 & 2.93 & 3.35 \\
Russian & 1.00 & 3.50 & 3.75  \\
Spanish & 1.00 & 3.10 & 3.05  \\
\hline
Average & 1.00 & 3.34 & 3.38 \\
\hline
\end{tabular}
 }
\caption{{\small Human Evaluation metrics on the generated samples. Samples are randomly drawn, and rated by the native speakers of Arabic, Chinese, Hindi, Russian and Spanish.}}
\label{tab:human_evals}
\end{table}

==> Multilingual QAGen/introduction.tex <==
\section{Introduction}
Generating question and answers from raw text has always been a challenging problem in natural language generation. Recently, there have been numerous efforts around question generation \cite{du2017learning,song-etal-2018-leveraging,klein2019learning,wangneural,ma2020improving,Chen2020Reinforcement,tuan2020capturing}.

Using such synthetic samples to improve the performance of question answering models has been explored by
\citet{puri2020nvidia}, \citet{alberti-etal-2019-synthetic}, and \citet{shakeri2020endtoend}, who show that reading comprehension (RC) models can be improved by generating large-scale synthetic training data. These promising results combined with the recent surge in the development of powerful generative models such as GPT-3 \cite{gpt3}, BART \cite{lewis2019bart}, and T5 \cite{raffel2019t5} suggest that the need for large manually labeled datasets can be reduced.

Although synthetic question-answer (QA) generation is well explored in English, the efficacy of such methods in the other languages remains an open question. Considering the lack of manually labeled QA datasets in many languages other than English, QA generation techniques can be applied to improve RC models in those languages. The emergence of multilingual generative models such as mBART \cite{mbart} and mT5 \cite{mt5} facilitates such endeavors.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Multilingual_QAGen.pdf}
    \caption{\small{End-to-End pipeline: 1)~Fine-tuning the generative model using SQuAD English samples and multilingual MLM\@. 2)~Generating synthetic samples from Wikipedia passages of the target language using the fine-tuned generative model. 3)~Training the downstream reading comprehension model using synthetic samples.}}
  \label{fig:pipeline}
\end{figure}

In this work, we propose generating multilingual question answer pairs to improve the performance of RC models in languages other than English. Besides unlabeled articles and questions, Our proposed method only requires labeled training samples in English, thus completely removing the need to acquire new labeled datasets. Our approach can easily be extended to any language, as long the multilingual generative model supports the language, and unlabeled questions and articles, such as Wikipedia, books, etc., exist in that language.

To enable zero-shot QA generation, the generative model should be able to produce non-English QA samples on non-English input when only trained on English samples. Inspired by the work of \citet{artetxe-etal-2020-cross,gururangan-etal-2020-dont,liu2020exploring}, we propose a multi-task learning setting, where during the fine-tuning stage, we train on two tasks in parallel: the target question-answer generation task, and the multilingual masked language modeling (MLM) task that was used in pre-training the generative model. Our experimental results show that including the MLM task is crucial in enabling the zero-shot capability of the fine-tuned generative model.



We propose fine-tuning a pre-trained multilingual T5 model on the SQuAD 1.1 \cite{squad11} training set. The fine-tuned model is then used to generate a large set of synthetic question-answer pairs from Wikipedia passages in the target language. Fig.~\ref{fig:pipeline} illustrates the end-to-end pipeline. We show that such synthetic samples can significantly boost RC models trained only on the English samples, with improvements up to 9 absolute points on F1\@. To summarize, our contributions are:

\begin{itemize}[topsep=3pt,itemsep=0ex,partopsep=1ex,parsep=1ex] % [noitemsep]
    % \itemsep1em 
    \item  Improving the zero-shot performance of multilingual RC models on multilingual QA tasks through generation of synthetic multilingual QA pairs.
    \item Proposing a multi-task fine-tuning of the multilingual generative model which is crucial in enabling zero-shot multilingual generation.
    \item Our approach is entirely zero-shot. No manually-labeled sample is used in fine-tuning of generative models on target languages, applicable to both high and low resource languages.
    \item Demonstrating grammatical correctness and sensibility of generated questions through human evaluations.
\end{itemize}

The rest of the paper is organized as follows. In section \ref{sec:e2e}, we discuss the process designed to train the generative model and produce synthetic samples. Section \ref{sec:related} discusses related work in the area of multilingual question-answer generation. In section \ref{sec:experiments}, we present experiments to measure the quality of generated samples. Section \ref{sec:downstream_experiments} focuses on the application of synthetic question-answer samples to downstream reading comprehension models. Finally, we conclude in section \ref{sec:conclusion}.

==> Multilingual QAGen/method.tex <==
\section{End-to-End Question-Answer Generation and Filtering}\label{sec:e2e}

\subsection{Modeling}\label{sec:modeling}
We use pre-trained ``multilingual T5'' (mT5) \cite{mt5} as our generative model. The mT5 model is based on T5 \cite{raffel2019t5}, which is an encoder-decoder sequence-to-sequence model.
\subsection{QA Generation Task}\label{sec:qa_gen_task}
We follow the probability distribution factorization suggested by \citet{shakeri2020endtoend}, where:
\begin{align*}
  p(Q,A | P) = p(Q | P) \times p(A | Q, P)
\end{align*}
Sampling from the above factorization is performed as follows:
\begin{align*}
    q \sim p(Q|P), a \sim p(A|Q,P) 
\end{align*}
where $Q,P,A$ refer to question, passage, and answer, respectively. 
During fine-tuning, passage tokens are fed as inputs, and the targets are a concatenation of the question and answer tokens.
During sampling, candidate passages are passed as inputs to the fine-tuned generative model, and question-answer pairs are sampled from the decoder.

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{Multitask_finetuning.pdf}
    \caption{\small{Multi-task fine-tuning of the multilingual pre-trained mT5 model: 1)~QA generation task, which uses SQuAD English samples, 2)~MLM task on a subset of mC4, 3)~MLM on the questions from the TyDiQA Gold Passage Task. The MLM variant used does not include sentinel tokens in the decoder output.}}
  \label{fig:model}
\end{figure*}

Fig.~\ref{fig:model} depicts the fine-tuning and sampling processes. We prepend \textit{``question''} to the question tokens and \textit{``answer''} to the answer tokens, to help the model distinguish one from the other.
\subsection{Masked Language Modeling Task}\label{sec:mlm}
The mT5 model is pre-trained on the large multilingual ``mC4'' dataset \cite{mt5} built from Common Crawl data, and trained using a Masked Language Modeling (MLM) task. This task involves replacing contiguous spans of input tokens with unique sentinel tokens (one per span). The decoder is then trained to reconstruct all the masked spans in the input, using a standard cross-entropy loss. We found a variant of this MLM task, where we remove all ``sentinel'' tokens (corresponding to non-masked spans in the input text) from the target sequence, as we notice this improves the quality of generated QAs. This variant is used in this work.

\subsection{Multi-Task Fine-Tuning}\label{sec:multi-task}
To perform zero-shot generation, the model needs to not only learn the QA Generation task, but also to retain its multilingual generation capabilities achieved during pre-training. To avoid \textit{catastrophic forgetting} \cite{FRENCH1999128}, which could lead to degraded generation capability, we propose a multi-task setting, where a predetermined percentage of fine-tuning examples comes from the QA Generation task, while the remaining examples (trained in parallel) are from a mixture of two MLM tasks: 1) MLM on a subset of mC4 which is a continuation of mT5 pre-training, 2) MLM on the questions from TyDiQA Gold Passage dev and training sets. The MLM on mC4 task helps the fine-tuned model retain its multi-lingual generation capabilities, while the MLM on TyDiQA questions task further improves the question generation capabilities of the generative model. Please note that the only supervised QA training data is SQuAD 1.1. The MLM task on TyDiQA questions is not conditioned on the associated passages of the questions. Experimental results in section \ref{sec:experiments} demonstrate the efficacy of this proposed approach. Fig.~\ref{fig:model} illustrates the multi-task fine-tuning process.

Fig.~\ref{fig:samples_multitask} demonstrates examples of generated samples in five languages using an mT5-XL (4B parameter) model fine-tuned in the multi-task setting (\ref{sec:multi-task}). It can be observed that: 1)~The generated questions are in the same language as the passage most of the time, 2)~The answers are relevant to the generated questions, 3)~The model is capable of generating long and non-trivial QA pairs.

% Comparing the samples in Figs.~\ref{fig:samples_multitask} and \ref{fig:samples_qa_gen} highlights the importance of including the MLM task (\ref{sec:mlm}) during fine-tuning to enable generation of questions in the target language. We observe that the model trained only on SQuAD samples fails to generated questions in the language of the target passage, and mostly generated English tokens. This is in contrast to the samples from the model that leverage MLM during fine-tuning. The samples are all generated in the language of the input passage.

Fig.~\ref{fig:samples_qa_gen} illustrates generated QA samples in Spanish and Arabic, when only the QA Generation task (\ref{sec:qa_gen_task}) is included in the fine-tuning. We observe: 1) Questions are primarily in English, not the target language, 2) Outputs contain certain tokens and entities mentioned in the language of the passage, 3) Ignoring language issues, the outputs exhibit semantically well-formed QA correspondence.


\subsection{Decoding and Filtering}\label{sec:filtering}

% We follow the \textit{sample and reranking} approach suggested by \citet{adiwardana2020humanlike}, where \textit{top-k} sampling is performed to generate multiple samples for each passage. The generated candidate samples are sorted decreasingly according to the language model score assigned to them by the generative model, and top samples are selected. This filtering approach based on likelihood score is referred to as \textit{likelihood filtering} \cite{shakeri2020endtoend}.

% Using the F1 score of a trained RC model to perform filtering, a.k.a.~\textit{round-trip} filtering, has been previously explored by \citet{puri2020training} and \citet{alberti-etal-2019-synthetic}. While it is shown to be effective, it adds extra complexity of running the RC model over the synthetic samples, and if the RC model is not accurate enough, it could filter out high quality and complicated samples, as suggested by \citet{shakeri2020endtoend}. This danger is amplified in target languages where the zero-shot performance of the RC model is low. For these reasons, we restrict attention to likelihood filtering in this work.

Since the accuracy of the generated question and answers is vital in improving the performance of downstream model, such generated samples require a strong filtering technique. Using the F1 score of a trained RC model to perform filtering, a.k.a.~\textit{round-trip} filtering, has been previously explored by \citet{puri2020training} and \citet{alberti-etal-2019-synthetic}. For a generated QA sample \textit{(q,~a,~p)}, where \textit{q}, \textit{a}, and \textit{p} indicate question, answer, and passage, the following steps are performed: 1) A trained RC model is applied to \textit{(q,~p)}, thus predicting \textit{$a'$}, and 2) The F1 score of \textit{a} and $a'$ is calculated, and if above a certain threshold, \textit{(q,~a,~p)} is kept, otherwise dropped.

 %4) Sometimes the generated question is entirely or partly in English, which we speculate to be an artifact of using only English samples in the QA Generation task. This introduces an inductive bias towards generation in English.
 
%  We asked native speakers of Russian and Spanish to evaluate the samples in Fig.~\ref{tab:samples_multitask}. The evaluation of the Russian samples indicates that the QAs are semantically correct except that the first question lacks the question word.
 
%  The Spanish assessment is that the questions are semantically correct, apart from the last question, which is in English. However, our consultant pointed out that the samples are robotic. We hypothesize that this stems from the fact that the QA Generation fine-tuning task does not including any samples in Spanish. Another issue with the Spanish samples is the lack of question mark at the beginning of the questions.
%  The automatic translations of QA samples in Fig. \ref{fig:samples_multitask} are included in Figs. \ref{tab:samples_multitask_1} and \ref{tab:samples_multitask_2} in the appendix. Public Google Translate service was used to convert the generated samples to English.
 
% \begin{table*}[ht]
% \centering
% \scriptsize
% \begin{tabular}{ll}
% \hline
% \multicolumn{2}{l}{}
% \begin{minipage}{15 cm}
% \textit{\textbf{Spanish}}\\ 
% Temprano en la mañana, cuando hay poco tráfico en las autopistas Tōmei y Chūō, el viaje entre Tokio y el lago Yamanaka toma una hora. El tráfico se vuelve pesado más tarde y el viaje toma un tiempo más largo. La ruta nacional de Japón 138 y la ruta nacional de Japón 413 corren a lo largo de las orillas del lago. Hay servicios de autobús disponibles desde la estación Fujisan ( línea Fujikyuko ), la estación JR Gotemba (línea JR Gotemba ) y la estación JR Mishima (JR Shinkansen ). Los servicios de autobuses de la autopista también están disponibles en la estación Shinjuku ( Tokio ).
%   \end{minipage} \hfill
%   \\
%   \\
%  Q: \textit{¿Cuánto tiempo se lleva entre Tokio y el lago Yamanaka?} & A: \textit{una hora}\\ 
%  \hline
% \multicolumn{2}{l}{}
% \begin{minipage}{15 cm}
% \textit{\textbf{Arabic}}\\ 
% \foreignlanguage{arabic}{ العلوم الطبية هي اختصاص طبي الذي يعتمد على إجراء التحاليل على السوائل الجسمية، وتحليل النتائج بشكل طبي في إطار تحديد الأصل الفيزيوبايولوجي لمرض ما .وهي دراسة بين علم الأمراض والتشريح المرضي. في معظم البلدان الناطقة بالفرنسية مصطلح العلوم الطبية غالبا ما يقصد به العلوم الطبية الحيوية .}
%   \end{minipage} \hfill
%   \\
%   \\
% Q:\foreignlanguage{arabic}{\textit{ وفي أي بلد يقصد به العلوم الطبية الحيوية ؟ }} & A:\foreignlanguage{arabic}{\textit{معظم البلدان الناطقة بالفرنسية}}
%  \\
% \hline
 
%   \multicolumn{2}{l}{}
% \begin{minipage}{15 cm}
% \textit{\textbf{Chinese}}\\ 
% 玩具总动员  《玩具总动员》（）是一部于1995年上映的美国计算机动画冒险喜剧片，由皮克斯动画工作室制作，华特迪士尼影业发行。该片是约翰·拉塞特的导演处女作，也是皮克斯制作的一部计算机动画长片和第一部剧场影片。影片的主角是一队在人类面前假装没有生命的拟人化玩具，侧重于提线牛仔玩偶（汤姆·汉克斯配音）和宇航员巴斯光年（提姆·艾伦配音）之间的关系。影片由约翰·拉塞特、安德鲁·斯坦顿、、和乔斯·韦登编剧，兰迪·纽曼配乐。史蒂夫·乔布斯和艾德文·卡特姆担纲执行制片人。影片于1995年11月22日在剧院上映。  为宣传他们的计算机而制作动画短片的皮克斯在以小玩具讲故事的短片《小锡兵》大获成功后，接触迪士尼，打算制造一部计算机动画长片。拉塞特、斯坦顿和皮特·多克特将先前写好的剧本大纲交给迪士尼，推动一部更前卫的电影。故事卷轴被毁灭后，制作被中断，剧本被重写，皮克斯所希望的“玩具深深希望孩子们能和它们一同玩耍，这种欲望驱动着它们的希望、恐惧和行动”的主题和基调得到更好地反映。工作室之后组建了一支员工相。
%   \end{minipage} \hfill
%   \\
%   \\
% Q: \textit{《玩具总动员》是什么类型的电影?} & A: \textit{美国计算机动画冒险喜剧片} \\
%  \hline
 
% \multicolumn{2}{l}{}
% \begin{minipage}{15 cm}
% \textit{\textbf{Russian}}
% \\
% \foreignlanguage{russian}{
% В местном кметстве Флорентин, в состав которого входит Флорентин, должность кмета (старосты) исполняет Любка Георгиева Константинова (коалиция в составе 2 партий: Болгарская социалистическая партия (БСП), Земледельческий союз Александра Стамболийского (ЗСАС)) по результатам выборов правления кметства.Кмет (мэр) общины Ново-Село — Георги Герасимов Стоенелов (независимый) по результатам выборов в правление общины.
% }
%   \end{minipage} \hfill \\ 
% \\
%  Q:\foreignlanguage{russian}{\textit{Кто управляет общиной Ново-Село?}} & A:\foreignlanguage{russian}{\textit{Георги Герасимов Стоенелов}}\\

%   \hline

%   \multicolumn{2}{l}{}
% \begin{minipage}{15 cm}
% \textit{\textbf{Hindi}}
%  \\
% % {
% % सिन्धी भाषा विधेयक, १९७२ पाकिस्तान के सिन्ध विधानसभा में १९७२ में प्रस्तुत एक विधेयक (बिल) था जिसे ३ जुलाई को तत्कालीन मुख्यमन्त्री मुमताज भुट्टो ने प्रस्तुत किया। इस विधेयक ने सिन्ध प्रान्त में सिन्धी भाषा को एकमात्र आधिकारिक भाषा घोषित कर दिया। इसके बाद ७ जुलाई से सिन्ध में भाषाई दंगे शुरू हो गये। तब पाकिस्तान के प्रधानमन्त्री जुल्फिकार अली भुट्टो ने घोषणा की कि उर्दू और सिन्धी दोनों ही सिन्ध की राजभाषाएँ होंगी। आधिकारिक रूप से सिन्धी को उर्दू के समकक्ष बनाये जाने से उर्दू बोलने वाले लोग निराश हो गये क्योंकि वे सिन्धी नहीं बोलते थे।
% % }
%  \end{minipage} \hfill \\
%  \\
%   \hdashline
% %  Q: \foreignlanguage{hindi}{\textit{किस भाषा को एकमात्र आधिकारिक भाषा घोषित कर दिया}? } & A:\foreignlanguage{hindi}{ \textit{सिन्धी}}
% \\ 
% \end{tabular}
% \caption{\small Samples of generated QAs in Spanish, Russian, Chinese, Arabic, and German. The generative model is mT5-XL fine-tuned on the mixture setting of Section \ref{sec:multi-task}. }
% \label{tab:samples_multitask}
% \end{table*}

\begin{figure*}[h]
    \centering
    \includegraphics[scale=0.25]{samples_original.png}
    \caption{\small Samples of generated QAs in Spanish, Russian, Chinese, Arabic, and German. The generative model is mT5-XL fine-tuned on the mixture setting of section~\ref{sec:multi-task}. \textbf{\textit{Trans.}} refers to translations of the QA sample using Google Translate service.} % \ref{sec:multi-task}.
  \label{fig:samples_multitask}
\end{figure*}

% \begin{figure*}[h!]
%     \centering
%     \includegraphics[scale=0.38]{samples_1.png}
%     \caption{\small {Samples of generated QAs in Spanish, Russian, Chinese, Arabic, and German. The generative model is mT5-XL fine-tuned on the co-training setting of Section \ref{sec:multi-task}.}}
%   \label{tab:samples_multitask}
% \end{figure*}

% \begin{table*}[ht]
% \centering
% \scriptsize
% \begin{tabular}{ll}
%  \hline
% \multicolumn{2}{l}{}
% \begin{minipage}{15 cm}
% \textit{\textbf{Spanish}}\\
%  Richard Anton Patrick Connel O'Ferrall (Paramaribo, 21 de julio 1855 - 28 de octubre de 1936) fue un maestro, escritor y miembro del Parlamento de Surinam. Durante la última década del siglo XIX y principios del siglo XX O'Ferrall fue una de las figuras centrales en la vida cultural de Paramaribo. Se graduó de maestro en holandés, francés e inglés y en 1881 escribió acerca de un método para la enseñanza de la lectura inicial. Fue director de una escuela especial para la Educación Primaria Avanzada (ULO) y también director de la puesta en marcha en 1888 de la escuela pública de formación de artesanos que publicó desde 1893 un catálogo de obras y tévnicas constructivas. Con los estudiantes de la clase más alta que formó el grupo teatral Ons Genoegen. Él escribió artículos para la revista De Ambachtsman (El Artesano), pero en ocasiones también para los periódicos locales.
%   \end{minipage} \hfill
%   \\
%  \hdashline
%  Q: \textit{Who was Richard Anton Patrick Connel O'Ferrall?} & A: \textit{maestro, escritor y miembro del Parlamento de Surinam}\\ 
%  Q: \textit{When did Richard O'Ferrall die?} & A:  \textit{28 de octubre de 1936} \\ 
%  Q: \textit{Where did Richard O'Ferrall live?} & A: \textit{Paramaribo} \\
%  \hline
%  \multicolumn{2}{l}{}
% \begin{minipage}{15 cm}
% \textit{\textbf{Arabic}}\\ 
% \foreignlanguage{arabic}{ آبلة (بالإسبانية:\foreignlanguage{english} {Ávila}) هي مدينة تقع في وسط إسبانيا، هي عاصمة مقاطعة آبلة التابعة لمنطقة قشتالة وليون.الديموغرافيا بلغ عدد سكان مدينة آبلة 59.008 نسمة عام 2011 (وفقاً للمعهد الوطني للإحصاء الإسباني).توأمة لآبلة اتفاقيات توأمة مع كل من: فيلنوف سور لوت روي-مالميزون تيرامو رودسأعلام توماس دي توركيمادا خيسوس هرنانديز أوبيدا سانتشث ألبورنوث فيليسيانو ريفيلا خيسوس هرنانديز جيل غونزاليس جيل غونزاليس دافيلا توماس لويس دي فيكتوريا كارلوس ساستري خوليو خيمينيزمراجعانظر أيضًا قائمة مواقع التراث العالمي في إسبانيا موقع التراث العالمي قائمة ...}
%   \end{minipage} \hfill
%   \\
%   \\
%  \hdashline
% Q:{\textit{Where is \foreignlanguage{arabic}{آبلة} located?}} & A:\foreignlanguage{arabic}{\textit{فوسط إسبانيا}}\\
% Q:\textit{How many people lived in \foreignlanguage{arabic}{آبلة} in 2011?}& A:\textit{59.008}  \\ 
% Q:{\textit{What is the number of inhabitants of the city of Ávila?}} & A:\textit{59.008} \\
%  \\
%  \hline
% \end{tabular}
% \caption{\small Samples of generated QAs in Spanish, and Arabic. The mT5-XL model is unable to generate valid questions in the target language, as in this case it was fine-tuned exclusively on the English QA Generation task from Section \ref{sec:qa_gen_task}.}
% \label{tab:samples_qa_gen}
% \end{table*}

\begin{figure*}[h]
    \centering
    \includegraphics[scale=0.28]{samples_en_only.png}
    \caption{\small Samples of generated QAs in Spanish and Arabic. The mT5-XL model is unable to generate valid questions in the target language, as in this case it was fine-tuned exclusively on the English QA generation task from section~\ref{sec:qa_gen_task}.}
  \label{fig:samples_qa_gen}
\end{figure*}

% \begin{figure*}[h!]
%     \centering
%     \includegraphics[scale=0.29]{samples_4.png}
%     \caption{\small {Samples of generated QAs in Spanish, and Arabic. The mT5-XL model is unable to generate valid questions in the target language, as in this case it was fine-tuned exclusively on the English QA Generation task from Section \ref{sec:qa_gen_task}.}}
%   \label{tab:samples_qa_gen}
% \end{figure*}

==> Multilingual QAGen/mlqa.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\scalebox{0.92}{
\begin{tabular}{l|ccccccccccccccccccc}
\hline
\multirow{2}{*}\textbf{Dataset} & \multicolumn{2}{c}{\textbf{ES}} & \multicolumn{2}{c}{\textbf{DE}} & \multicolumn{2}{c}{\textbf{AR}} &
\multicolumn{2}{c}{\textbf{HI}} & \multicolumn{2}{c}{\textbf{VI}} & \multicolumn{2}{c}{\textbf{ZH}} \\ 
& EM & F1 & EM & F1 & EM & F1 & EM & F1 & EM & F1 & EM & F1 \\
\hline
SQuAD en &47.42 & 65.10 & 44.65 & 59.62& 33.06 & 51.27 & 34.83 &50.30 &41.53 & 61.51 &38.70 & 59.14\\ 
Synthetic only &48.81 & 67.58 & 46.96 & 63.17 & 35.50 & 54.62 &40.02 & 58.01 &42.88&63.15 &34.55 & 59.20\\
SQuAD en + Synth. &\textbf{51.70}&\textbf{70.32} & \textbf{49.63} & \textbf{65.21} &\textbf{37.71}& \textbf{56.48} & \textbf{42.94}& \textbf{59.96} & \textbf{46.02}& \textbf{66.79}  & \textbf{42.20}& \textbf{64.19}\\ 
\hdashline
\textit{Supervised} & 52.90 & 70.74 & 51.36 & 65.86 & 38.76 & 57.88 & 45.69 & 62.72 & 47.28 & 67.57 & 43.84 & 65.98 \\
\hline
\end{tabular}
}
\caption{{\small Performance of fine-tuned mBERT models on MLQA test set. \textit{Supervised} refers to training on SQuAD en + \texttt{translate-train} dataset of the target language.}}\label{tab:mlqa}
\end{table*}

==> Multilingual QAGen/qgen.tex <==
\begin{table}[]
\centering
\footnotesize
\scalebox{0.85}{
\begin{tabular}{l|rrrrrrr} \hline
Training Task          & ar  & de   & en   & es  & hi  & vi   & zh  \\ \hline
SQuAD en & 1.7 & 3.0  & 23.4 & 3.6 & 3.2 & 4.4  & 1.2 \\
Mixture 1 & 12.2&	14.9&	25.0 & 18.4&	10.6&	13.8&	10.0 \\ 
Mixture 2 & 13.1 & 15.2 & 24.9 & 18.4 & 11.1 & 13.9 & 9.7 \\ 
Mixture 3 & 14.5 & 14.8 & 25.0 & 18.6 & 10.8 & 13.5 & 9.6 \\ \hline
\end{tabular}
}
\caption{{\small Comparison of question generation quality (BLEU score) on the MLQA test set with mT5-XL: The Mixtures are as follows: \textit{SQuAD en}: SQuAD en as the training data, \textit{Mixture 1}: SQuAD en + MLM on mC4 subset, \textit{Mixture 2}: SQuAD en + TyDiQA questions, \textit{Mixture 3}: SQuAD en + MLM on mC4 subset + MLM on TyDiQA questions. }}
\label{qgen}
\end{table}

==> Multilingual QAGen/qgen_size.tex <==
\begin{table}[]
\centering
\footnotesize
\scalebox{0.86}{
\begin{tabular}{l|rrrrrrr} \hline
Model Size     & ar  & de   & en   & es  & hi  & vi   & zh  \\  \hline
Base (600M)  & 3.9 & 5.1  & 19.0 & 8.2 & 3.5 & 7.4  & 3.1 \\ 
Large (1B) & 10.3 & 5.7  & 23.9 & 5.9 & 4.3 & 6.2  & 3.9 \\
XL (4B)   & 14.5 & 14.8 & \textbf{25.0} & 18.6 & 10.8 & 13.5 & 9.6 \\
XXL (13B)   & \textbf{15.8} & \textbf{16.2} & \textbf{24.9} & \textbf{19.3} & \textbf{12.2} & \textbf{15.6} & \textbf{10.2} \\
\hline
\end{tabular}
}
\caption{{\small Performance of question generation (mixture setting) on the MLQA test set for different mT5 model sizes.}}
\label{qgen-size}
\end{table}

==> Multilingual QAGen/related_work.tex <==
\section{Related Work}\label{sec:related}
Recent work has explored question-answer generation \cite{alberti-etal-2019-synthetic, puri2020training, lee2020generating,shakeri2020endtoend}, but limited in scope to English. We leverage the modeling and filtering approaches proposed by \citet{shakeri2020endtoend} due to their simplicity and effectiveness.

\citet{cross-ling-training} explores cross lingual question generation. In contrast to our work, this only generates questions, without the corresponding answers. Additionally, this approach requires a complicated pre-training process on the target languages, as well as gold samples to fine-tune the generative models, so it is not easily extensible to other languages. This is in contrast to our work, which does not require any gold QA samples in any language other than English. Another distinguishing factor is that we demonstrate improved performance on downstream QA tasks, while \citet{cross-ling-training} only measure the quality of the generated samples on automatic metrics such as BLEU, and human evaluations.

Similarly, \citet{chi2019crosslingual} explore cross-lingual question-only generation using SQuAD English samples. They propose cross-lingual pre-training on the source and target languages. Similar to \citet{cross-ling-training}, their focus is only on the quality of the generated questions, whereas we validate our approach directly through improvements on downstream QA tasks. Moreover, while \citet{chi2019crosslingual} depends on a complex pre-training recipe and parallel sentences in both source and target languages, our approach not only does not require such parallel corpus, but also the MLM task included in our fine-tuning setting is widely used and studied. This leads to our approach being more easily adaptable to other languages and pre-trained generative models.

Most closely related to our work is the multilingual synthetic question generation approach of \citet{riabi2020synthetic}. However, there are two important differences between the two approaches. Firstly, our work includes both question and answer generation using a single model, while theirs only focuses on question generation. We believe generating the question and answer jointly is a richer problem that better harnesses the capabilities of pre-trained language models. Their question generation is conditioned on the selected answers, which further limits the generation. Secondly, their proposed method depends on translated SQuAD to target languages to fine-tune the generative model, hence limiting the application of their approach to languages that such translation data does not exist. Even if such translated data exists in a target language, the quality of the samples generated by the generative model trained on such training data is highly affected by the quality of the translations. This could lead to low quality QA samples in low resource languages.  This is in contrast to our zero-shot approach, which does not require any training data in the target language.

==> Multilingual QAGen/tydiqa.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\scalebox{0.92}{
\begin{tabular}{l|ccccccccccccccccccc}
\hline
\multirow{2}{*}\textbf{Dataset} & \multicolumn{2}{c}{\textbf{AR}} & \multicolumn{2}{c}{\textbf{RU}} & \multicolumn{2}{c}{\textbf{FI}} & \multicolumn{2}{c}{\textbf{TE}}\\ 
& EM & F1 & EM & F1 & EM & F1 & EM & F1\\
\hline
SQuAD en &45.39& 60.93 & 40.52 & 63.07 & 45.27 & 58.91 & 45.44 & 53.73  \\ 
Synthetic only &\textbf{56.35}& \textbf{71.85}& \textbf{40.52}& \textbf{67.09} & 62.28 & 74.44 & \textbf{46.04} & \textbf{59.12}  \\
SQuAD en + Synth. &55.81& 71.52 & \textit{39.66}& \textit{66.70} & \textbf{62.79} & \textbf{74.74} & 45.44 & 54.58 \\
\hdashline
\textit{Supervised} & 67.75 & 82.46 & 59.36 & 76.03 & 69.69 & 80.65 & 70.55 & 84.74 \\
\hline
\end{tabular}
}
\caption{{\small Performance of fine-tuned QA models on TyDiQA Gold Passage task. \textit{Supervised} refers to train on TyDiQA Gold Passage training data.}}\label{tab:tydiqa}
\end{table*}

==> Multilingual QAGen/xquad.tex <==
\begin{table*}[]
\centering
\footnotesize
\scalebox{0.92}{
\begin{tabular}{l|ccccccccccccccccccc}
\hline
\multirow{2}{*}\textbf{Dataset} & \multicolumn{2}{c}{\textbf{ES}} & \multicolumn{2}{c}{\textbf{DE}} & \multicolumn{2}{c}{\textbf{AR}} &
\multicolumn{2}{c}{\textbf{HI}} & \multicolumn{2}{c}{\textbf{VI}} & \multicolumn{2}{c}{\textbf{ZH}} \\ 
& EM & F1 & EM & F1 & EM & F1 & EM & F1 & EM & F1 & EM & F1 \\
\hline
SQuAD en  & 57.06 & 74.62 & 55.55 & 71.46 & 43.28 & 60.26 & 44.62 & 59.21 & 50.84 & 70.66 & 50.59 & 59.07\\ 
Synthetic only & 57.90 & 75.43 &54.79 & 72.06 & 45.38 & 62.57 & 46.13 & 62.57 & 49.33 & 68.25 & 42.86 & 58.70\\
SQuAD en + Synth. & \textbf{60.50} & \textbf{78.50} & \textbf{59.41} & \textbf{75.36} & \textbf{49.33} & \textbf{66.00} &\textbf{50.17} & \textbf{66.24} &\textbf{53.45} & \textbf{73.12} & \textbf{52.27} & \textbf{63.32}\\ 
\hdashline
\textit{Supervised} & 63.87 & 80.61 & 62.10 & 76.99 & 54.79 & 70.85 & 56.13 & 70.86 & 58.57 & 77.35 & 58.99 & 67.02\\
\hline
\end{tabular}
}
\caption{{\small Performance of fine-tuned mBERT models on XQuAD. \textit{Supervised} refers to training on SQuAD en + \texttt{translate-train} dataset of the target language.}}\label{tab:xquad}
\end{table*}




==> Multilingual QAGen/xquad_mt5_base.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\scalebox{0.95}{
\begin{tabular}{l|cccccccccccc}
\hline
% \textbf{Dataset} & \textbf{ES}\textbf{DE}\textbf{AR} &
% \textbf{HI} & \textbf{VI}\textbf{ZH} \\ 
\textbf{Dataset} & en & ar & de & el & es & hi & ru & th & tr & vi & zh & avg \\
\hline
SQuAD en (paper) & 84.6  & 63.8 & 73.8  & 59.6 & 74.8 & 60.3  & 57.8 & 57.6  & 67.9  & 70.7 & 66.1  & 67.0 \\ \hdashline
SQuAD en (ours) & \textbf{85.5} & 65.7 & 73.6 & 62.5 & 75.0 & 62.4& 61.9 & 57.6 & 68.9 & \textbf{71.9} & \textbf{71.1} & 68.1 \\
SQuAD en + ru & 83.7& 67.5 & 73.6 & 69.3 & 73.8 & \textbf{66.2} & 70.3 & 62.7 & 67.5 & 68.8 & 68.9 & 70.0 \\
SQuAD en + hi & 84.2 & 68.3 & 75.0 & 68.4 & 75.0 & 63.7 & 68.2 & \textbf{64.5} & 67.2 & 69.5 & 68.9 & 69.9 \\
SQuAD en + de & 84.6& \textbf{69.0} & 71.8 & \textbf{70.2} & \textbf{75.7} & \textbf{66.2} & \textbf{71.0} & 63.5 & \textbf{70.0} & 70.9& \textbf{71.2} & \textbf{71.0} \\
SQuAD en + ar & 84.5& 64.0& 74.4& 69.4& 74.4 & 65.1 & 65.1 & 62.5 & 67.9 & 70.0 & 70.2 & 70.2 \\
SQuAD en + es & 84.8 & \textbf{69.1} & \textbf{76.1} & 68.2 & 72.8 & 65.4 & 68.9 & 62.7 & 70.0 & 71.0 & 71.0 & 70.6 \\
\hline
Supervised & 83.1 & 72.4 & 76.9 & 76.8 & 79.0 & 71.4 & 76.1 & 67.9 & 72.5 & 75.9 & 76.9 & 75.3 \\
% Synthetic only & 57.90 & 75.43 &54.79 & 72.06 & 45.38 & 62.57 & 46.13 & 62.57 & 49.33 & 68.25 & 42.86 & 58.70\\
% SQuAD en + Synth. & \textbf{60.50} & \textbf{78.50} & \textbf{59.41} & \textbf{75.36} & \textbf{49.33} & \textbf{66.00} &\textbf{50.17} & \textbf{66.24} &\textbf{53.45} & \textbf{73.12} & \textbf{52.27} & \textbf{63.32}\\ 
% \hdashline
% \textit{Supervised} & 63.87 & 80.61 & 62.10 & 76.99 & 54.79 & 70.85 & 56.13 & 70.86 & 58.57 & 77.35 & 58.99 & 67.02\\
\hline
\end{tabular}
}
\caption{{\small Performance of fine-tuned mT5 Base models on XQuAD. \textit{Supervised} refers to training on SQuAD en + \texttt{translate-train} dataset of the target language.}}\label{tab:xquad_mt5_base}
\end{table*}

==> Multilingual QAGen/xquad_mt5_large.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\scalebox{0.95}{
\begin{tabular}{l|cccccccccccc}
\hline
% \textbf{Dataset} & \textbf{ES}\textbf{DE}\textbf{AR} &
% \textbf{HI} & \textbf{VI}\textbf{ZH} \\ 
\textbf{Dataset} & en & ar & de & el & es & hi & ru & th & tr & vi & zh & avg \\
\hline
SQuAD en (paper) & 88.4 &  75.2 & 80.0 & 77.5 & 81.8 & 73.4 & 74.7 & 73.4 & 76.5 & 79.4 & 75.9 & 77.8 \\ \hdashline
SQuAD en (ours) & 88.6 & 75.0 & 80.4 & 76.5 & 81.6 & 73.9 & 74.1 & 73.8 & \textbf{76.2} & \textbf{80.1} & 76.4 & 77.4 \\
SQuAD en + ru & 88.2 & 76.6 & 81.2 & 79.1 & 82.6 & 76.1 & 77.6 & 72.1 & 75.1 & 78.4 & 77.4 & \textbf{78.6} \\
SQuAD en + hi & \textbf{88.9} & 76.7 & 81.5 & 79.4 & \textbf{82.9} & 73.4 & 78.7 & \textbf{74.1} & 75.0 & 79.1 & 78.0 & \textbf{78.6} \\
SQuAD en + de & 88.0 & 72.7 & 79.7 & 73.0 & 82.0 & 73.6 & 76.4 & 71.6 & 74.8 & 78.7 & 76.2 & 76.6 \\
SQuAD en + ar & 88.0 & 73.3 & 81.2 & 78.8 & 82.4 & 75.1 & 78.5 & 71.4 & 75.6 & 77.3 & \textbf{78.2} & 77.8 \\
SQuAD en + es & 88.2 & \textbf{77.2} & \textbf{81.8} & \textbf{79.9} & 81.3 & \textbf{76.4} & \textbf{79.2} & 72.3 & 75.8 & 79.5 & 77.7 & \textbf{78.7} \\
\hline
Supervised & 87.3 & 79.4 & 82.7 & 81.8 & 83.8 & 78.0 & 81.9 & 74.7 & 80.2 & 80.4 & 83.2 & 81.2 \\
% Synthetic only & 57.90 & 75.43 &54.79 & 72.06 & 45.38 & 62.57 & 46.13 & 62.57 & 49.33 & 68.25 & 42.86 & 58.70\\
% SQuAD en + Synth. & \textbf{60.50} & \textbf{78.50} & \textbf{59.41} & \textbf{75.36} & \textbf{49.33} & \textbf{66.00} &\textbf{50.17} & \textbf{66.24} &\textbf{53.45} & \textbf{73.12} & \textbf{52.27} & \textbf{63.32}\\ 
% \hdashline
% \textit{Supervised} & 63.87 & 80.61 & 62.10 & 76.99 & 54.79 & 70.85 & 56.13 & 70.86 & 58.57 & 77.35 & 58.99 & 67.02\\
\hline
\end{tabular}
}
\caption{{\small Performance of fine-tuned mT5 Large models on XQuAD. \textit{Supervised} refers to training on SQuAD en + \texttt{translate-train} dataset of the target language.}}\label{tab:xquad_mt5_large}
\end{table*}

==> Multilingual QAGen/xquad_mt5_xl.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\scalebox{0.95}{
\begin{tabular}{l|cccccccccccc}
\hline
% \textbf{Dataset} & \textbf{ES}\textbf{DE}\textbf{AR} &
% \textbf{HI} & \textbf{VI}\textbf{ZH} \\ 
\textbf{Dataset} & en & ar & de & el & es & hi & ru & th & tr & vi & zh & avg \\
\hline
SQuAD en (paper) & 88.8 & 77.4 & 80.4 & 80.4 & 82.7 & 76.1 & 76.2 & 74.2 & 77.7 & 80.5 & 80.5 & 79.5  \\ \hdashline
SQuAD en (ours) & \textbf{89.7} & \textbf{79.2} & 80.9 & 80.9 & 83.2 & \textbf{78.7} & 78.4 & 74.3 & 78.4 & 79.5 & \textbf{80.7} & \textbf{80.2} \\
SQuAD en + ru & 89.1 & 78.6 & \textbf{82.1} & \textbf{81.7} & 82.7 & 78.6 & 79.4 & 74.3 & \textbf{78.7} & 80.6 & 79.2 & \textbf{80.2} \\
SQuAD en + hi & 89.1 & \textbf{79.1} & 81.7 & 80.9 & \textbf{83.4} & 76.1 & 79.0 & \textbf{74.6} & 77.6 & 81.0 & 80.4 & 79.9 \\
SQuAD en + de & 88.8 & 78.2 & 81.2 & \textbf{81.7} & 82.8 & 78.1 & \textbf{79.6} & 74.0 & 77.7 & \textbf{81.2} & 79.7 & 80.1 \\
SQuAD en + ar & 89.0 & 75.0 & 81.3 & 81.5 & 82.8 & 78.4 & 79.3 & 73.5 & 78.4 & 80.2 & 80.4 & 79.6 \\
SQuAD en + es & 88.8 & 79.0 & \textbf{82.2} & 81.3 & 82.6 & \textbf{78.7} & 78.8 & 73.8 & 78.3 & \textbf{81.1} & 80.5 & \textbf{80.2} \\
\hline
Supervised & 88.5 & 80.9 & 83.4 & 83.6 & 84.9 & 79.6 & 82.7 & 78.5 & 82.4 & 82.4 & 83.2 & 82.7  \\
\hline
\end{tabular}
}
\caption{{\small Performance of fine-tuned mT5 XL models on XQuAD. \textit{Supervised} refers to training on SQuAD en + \texttt{translate-train} dataset of the target language.}}\label{tab:xquad_mt5_xl}
\end{table*}

==> mlqa.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\scalebox{0.92}{
\begin{tabular}{l|ccccccccccccccccccc}
\hline
\multirow{2}{*}\textbf{Dataset} & \multicolumn{2}{c}{\textbf{ES}} & \multicolumn{2}{c}{\textbf{DE}} & \multicolumn{2}{c}{\textbf{AR}} &
\multicolumn{2}{c}{\textbf{HI}} & \multicolumn{2}{c}{\textbf{VI}} & \multicolumn{2}{c}{\textbf{ZH}} \\ 
& EM & F1 & EM & F1 & EM & F1 & EM & F1 & EM & F1 & EM & F1 \\
\hline
SQuAD en &47.42 & 65.10 & 44.65 & 59.62& 33.06 & 51.27 & 34.83 &50.30 &41.53 & 61.51 &38.70 & 59.14\\ 
Synthetic only &48.81 & 67.58 & 46.96 & 63.17 & 35.50 & 54.62 &40.02 & 58.01 &42.88&63.15 &34.55 & 59.20\\
SQuAD en + Synth. &\textbf{51.70}&\textbf{70.32} & \textbf{49.63} & \textbf{65.21} &\textbf{37.71}& \textbf{56.48} & \textbf{42.94}& \textbf{59.96} & \textbf{46.02}& \textbf{66.79}  & \textbf{42.20}& \textbf{64.19}\\ 
\hdashline
\textit{Supervised} & 52.90 & 70.74 & 51.36 & 65.86 & 38.76 & 57.88 & 45.69 & 62.72 & 47.28 & 67.57 & 43.84 & 65.98 \\
\hline
\end{tabular}
}
\caption{{\small Performance of fine-tuned mBERT models on MLQA test set. \textit{Supervised} refers to training on SQuAD en + \texttt{translate-train} dataset of the target language.}}\label{tab:mlqa}
\end{table*}

==> tydiqa.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\scalebox{0.92}{
\begin{tabular}{l|ccccccccccccccccccc}
\hline
\multirow{2}{*}\textbf{Dataset} & \multicolumn{2}{c}{\textbf{AR}} & \multicolumn{2}{c}{\textbf{RU}} & \multicolumn{2}{c}{\textbf{FI}} & \multicolumn{2}{c}{\textbf{TE}}\\ 
& EM & F1 & EM & F1 & EM & F1 & EM & F1\\
\hline
SQuAD en &45.39& 60.93 & 40.52 & 63.07 & 45.27 & 58.91 & 45.44 & 53.73  \\ 
Synthetic only &\textbf{56.35}& \textbf{71.85}& \textbf{40.52}& \textbf{67.09} & 62.28 & 74.44 & \textbf{46.04} & \textbf{59.12}  \\
SQuAD en + Synth. &55.81& 71.52 & \textit{39.66}& \textit{66.70} & \textbf{62.79} & \textbf{74.74} & 45.44 & 54.58 \\
\hdashline
\textit{Supervised} & 67.75 & 82.46 & 59.36 & 76.03 & 69.69 & 80.65 & 70.55 & 84.74 \\
\hline
\end{tabular}
}
\caption{{\small Performance of fine-tuned QA models on TyDiQA Gold Passage task. \textit{Supervised} refers to train on TyDiQA Gold Passage training data.}}\label{tab:tydiqa}
\end{table*}

==> xquad.tex <==
\begin{table*}[]
\centering
\footnotesize
\scalebox{0.92}{
\begin{tabular}{l|ccccccccccccccccccc}
\hline
\multirow{2}{*}\textbf{Dataset} & \multicolumn{2}{c}{\textbf{ES}} & \multicolumn{2}{c}{\textbf{DE}} & \multicolumn{2}{c}{\textbf{AR}} &
\multicolumn{2}{c}{\textbf{HI}} & \multicolumn{2}{c}{\textbf{VI}} & \multicolumn{2}{c}{\textbf{ZH}} \\ 
& EM & F1 & EM & F1 & EM & F1 & EM & F1 & EM & F1 & EM & F1 \\
\hline
SQuAD en  & 57.06 & 74.62 & 55.55 & 71.46 & 43.28 & 60.26 & 44.62 & 59.21 & 50.84 & 70.66 & 50.59 & 59.07\\ 
Synthetic only & 57.90 & 75.43 &54.79 & 72.06 & 45.38 & 62.57 & 46.13 & 62.57 & 49.33 & 68.25 & 42.86 & 58.70\\
SQuAD en + Synth. & \textbf{60.50} & \textbf{78.50} & \textbf{59.41} & \textbf{75.36} & \textbf{49.33} & \textbf{66.00} &\textbf{50.17} & \textbf{66.24} &\textbf{53.45} & \textbf{73.12} & \textbf{52.27} & \textbf{63.32}\\ 
\hdashline
\textit{Supervised} & 63.87 & 80.61 & 62.10 & 76.99 & 54.79 & 70.85 & 56.13 & 70.86 & 58.57 & 77.35 & 58.99 & 67.02\\
\hline
\end{tabular}
}
\caption{{\small Performance of fine-tuned mBERT models on XQuAD. \textit{Supervised} refers to training on SQuAD en + \texttt{translate-train} dataset of the target language.}}\label{tab:xquad}
\end{table*}



